Users are Closer than they Appear: Protecting User Location from WiFi APs

WiFi-based indoor localization has now matured for over a decade. Most of the current localization algorithms rely on the WiFi access points (APs) in the enterprise network to localize the WiFi user accurately. Thus, the WiFi user's location information could be easily snooped by an attacker listening through a compromised WiFi AP. With indoor localization and navigation being the next step towards automation, it is important to give users the capability to defend against such attacks. In this paper, we present MIRAGE, a system that can utilize the downlink physical layer information to create a defense against an attacker snooping on a WiFi user's location information. MIRAGE achieves this by utilizing the beamforming capability of the transmitter that is already part of the WiFi protocols. With this initial idea, we have demonstrated that the user can obfuscate his/her location from the WiFi AP always with no compromise to the throughput of the existing WiFi communication system and reduce the user location accuracy of the attacker from 2.3m to more than 10m.

==> design/design-3.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}

In this section, we first illustrate an attack model which will violate the Wi-Fi user's location privacy. We then propose on how a straightforward idea of beam nulling to the direct path to protect the user's privacy comes at the cost of user's throughput degradation. Finally, we propose the design of \name for Wi-Fi user's location obfuscation, which makes the reflected path appear to be the direct path.

\subsection{Attack Model} 
The attacking Wi-Fi APs in an enterprise network (say a shopping mall) listen to the channel transmitted by the user and predict the user directions to each of the APs using state-of-the-art AoA algorithms (say SpotFi~\cite{spotfi}). The APs can use the AoAs either for
(a)`single-AP Localization' by using the ToF measurements (from Wi-Peep~\cite{wipeep} for example) for range and estimated AoA for direction, or (b) `Triangulation' by using AoAs across multiple APs to estimate user location. The AoA of the incoming Wi-Fi signal at the attacking AP can be extracted via Spotfi~\cite{spotfi} as shown in Fig.~\ref{fig:profiles}(a). As discussed, the direct path (green box) arrives earlier than the reflected path (blue box) and hence direct path's AoA can be reliably extracted even in multipath-rich environments. 


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/results.pdf}
    \caption{Angle-Distance profiles representing the direct path and reflected path angle of arrivals and their relative distance travelled. Measurement from COTS AP in (a) without \name, in (b) with nulling the direct path, in (c) with \name obfuscation applied.}
    \label{fig:profiles}
\end{figure}


\subsection{Nulling to the Direct Path}~\label{sub:nulling}

Hence, to obfuscate the AoA information at the Wi-Fi user, a straightforward idea is to null this direct path to the AP. That is the user can beamform such that there is a null in the beampattern in the direction of AP's direct path. Now the attacker Wi-Fi AP will only observe the multipath and regard it as the direct path for localization. To perform this nulling, the Wi-Fi user extracts the AoA of direct path (i.e., $\theta_d$) and AoA of the earliest reflected path (i.e., $\theta_r$) from a downlink (AP to user) channel measurement. For the sake of simplicity, we only consider two paths. To null the direct path, the Wi-Fi user needs to apply the beamforming weights $N_d(f_i,k)$ to their data streams to null in the $\theta_d$ direction, where $i$ indicates the subcarrier index and $k$ indicates the antenna index. After we `precode' the data stream $X(f_i, k)$ with nulling weights, the Wi-Fi AP will receive the following signals:
\begin{align*}
    Y(f_i,k) &=H(f_i,k)N_d(f_i, k)X(f_i,k)\\
             &=(H_d(f_i, k)+H_r(f_i,k))N_d(f_i, k)X(f_i,k)\\
             &= H_r(f_i,k)N_d(f_i, k)X(f_i,k)
\end{align*}
where $Y(f_i,k)$ and $H(f_i,k)$ indicate the received signal and wireless channel on $k$-th antenna and $f_i$ subcarrier. $H(f_i,k)=H_d(f_k, k)+H_r(f_i,k)$ where $H_d$ and $H_r$ indicate the direct path and  reflected path wireless channel. Note that $H_d(f_i, k)N_d(f_i,k)=0$ as $N_d(f_i,k)$ is chosen to lie in the null space of $H_d(f_i, k)$ \cite{li2005null}. The Wi-Fi AP will estimate the wireless channel as $H_r(f_i,k)N_d(f_i, k)$, which only contains the reflected path, thereby preventing the attacker from extracting the direct path AoA. 

This is illustrated in the angle-distance profile in Fig.~\ref{fig:profiles}(b). Note the reduced power of the direct path. However, this simple idea has two key flaws. First, nulling to the direct path will decrease the signal strength at the Wi-Fi AP and degrade the network throughput. Second, in case the nulling angle is predicted incorrectly by the user, nulling will be ineffective and a residual peak of the direct path will remain exposing the user's location. Clearly, this solution is impractical and we propose \name for user location obfuscation to eliminate this side-effect.

\subsection{Beamforming and Delaying}\label{sec:mirage-des}

To overcome this user's throughput degradation we need to ensure the direct path is preserved, as direct-path contributes to majority of the channel diversity. However the presence of the direct path will appear as a strong signal at the Wi-Fi AP and an attacker can easily extract the AoA. However, to disambiguate the effects of the inevitable reflected paths, the attacker relies on the simple heuristic that the direct path always travels the shortest path. Specifically, for a distance travelled $d$, the phases accumulated across the various subcarriers are given by $e^{-2\pi f_c \frac{d}{c}}$. By leveraging super-resolution localization algorithms~\cite{spotfi}, the attacker can hence separate the various paths in the time-domain and predict the direct path. 

Here we provide a key insight -- delaying only the direct path signal invalidates the foundational heuristic to select the correct AoA. With this in mind, we propose to beamform to direct path and multipath and add delay to the direct path. This ensures communication throughput will be preserved over the beamforming and the user's location will be obfuscated through adding the delay to the direct path. This is qualitatively illustrated in Fig.~\ref{fig:profiles}(c). The Wi-Fi user adds a delay of $15$ m in the direction of the direct path and successfully pushes the direct path peak (green box) predicted by SpotFi to the right of the multipath peak (blue box).    

\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.40\linewidth}
    \includegraphics[width=\linewidth]{figures/setup.pdf}
    \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \begin{tabular}{|c|c|c|cccc|}
        \hline
        \multirow{2}{*}{} &
          \multirow{2}{*}{No obf.} &
          \multirow{2}{*}{Nulling} &
          \multicolumn{4}{c|}{\name with delay of} \\ \cline{4-7} 
         &  &  & \multicolumn{1}{c|}{0 (m)} & \multicolumn{1}{c|}{20 (m)} & \multicolumn{1}{c|}{30 (m)} & 40 (m) \\ \hline
        AoA error &
          $0^\circ$ &
          $62^\circ$ &
          \multicolumn{1}{c|}{$0^\circ$} &
          \multicolumn{1}{c|}{$58^\circ$} &
          \multicolumn{1}{c|}{$61^\circ$} &
          $53^\circ$ \\ \hline
        \begin{tabular}[c]{@{}c@{}}RSSI\\ (dBm)\end{tabular} &
          -65 &
          -71 &
          \multicolumn{1}{c|}{-64} &
          \multicolumn{1}{c|}{-64} &
          \multicolumn{1}{c|}{-64} &
          -62 \\ \hline
        \end{tabular}
        \subcaption{}
        \label{table:aoa_rssi}
    \end{minipage}
    \caption{\textbf{(a)} Hardware setup showcasing the ASUS WiFi-AP, WARP client and reflector. (b) AoA error and RSSI measured without obfuscation; with nulling; and using \name to delay the path by varying amounts}
    \label{fig:example-result}
\end{figure*}


Specifically, to beamform to the direct path and multipath, we need to have the beamforming vector $S_d(f_i,k)$ and $S_r(f_i,k)$ for the direct path and reflected path respectively~\cite{beam_forming_doc}. The specific beamforming angles are predicted via a downlink channel measurement at the user. Hence, the Wi-Fi user will use the precoding weight of $S_d(f_i,k)e^{-j2\pi f_i d_\mathrm{obf}/c}+S_r(f_i,k)$, where $d_\mathrm{obf}$ indicates the additional path length that Wi-Fi user wants to add to obfuscate its location for Wi-Fi AP as shown in Fig.~\ref{fig:mirage-idea}(d). We ensure that $d_\mathrm{obf} > d_\mathrm{multipath} - d_\mathrm{direct}$ via the same downlink channel measurements. Then, the Wi-Fi AP will receive the following signals:
\begin{align}
\label{eq:beam:delay}
     Y(f_i, k)&=H(f_i,k)(S_d(f_i,k)e^{-j2\pi f_i \frac{d_\mathrm{obf}}{c}} + S_r(f_i,k))X(f_i,k)\nonumber \\
             &=(H_d(f_k, k)+H_r(f_i,k))(S_d(f_i,k)e^{-j2\pi f_i\frac{d_\mathrm{obf}}{c}}\nonumber \\
             & \quad \quad \quad \quad  + S_r(f_i,k))X(f_i,k)\nonumber\\
             &=(H_d(f_k, k)S_d(f_i,k)e^{-j2\pi f_i\frac{d_\mathrm{obf}}{c}} \nonumber\\
             & \quad \quad \quad \quad + H_r(f_i,k)S_r(f_i,k))X(f_i,k)
\end{align}
% Beamforming in the directions of the direct path ensures weaker energy directed towards strongest multipath and vice versa. Hence, in Eqn.~\ref{eq:beam:delay}, the cross terms $H_d(f_k, k)S_r(f_i,k)$ and $H_r(f_i,k)S_d(f_i,k)e^{-j2\pi f_i d_\mathrm{obf}/c}$ are ignored. Thus, the wireless channel is $H_d(f_k, k)S_d(f_i,k)e^{-j2\pi f_i d_\mathrm{obf}/c}+H_r(f_i,k)S_r(f_i,k)$, which will only contain direct path with delay of $d_\mathrm{obf}$ and multipath without any delay. 


\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/discussion.pdf}
    \vspace{1pt}
    \caption{Imperfect beamforming introduces residual peak in angle-distance profile (red dotted box) due to the power leakage from the side lobe of the direct path beamforming. \textit{(left inset)} Antenna beamforming patterns transmitted by the user; \textit{right inset} received SpotFi profile at a commodity Wi-Fi AP}
    \label{fig:beam_null_mot}
\end{figure*}

\noindent\textbf{Problem of Imperfect Beamforming:}
We have demonstrated \name's obfuscation for the Wi-Fi user's location through beamforming and delaying through a few examples. However in \name's design we make a critical assumption. We ignore the cross terms in Eqn.~\ref{eq:beam:delay} when adding delay to the direct path due to weaker energy directed towards the reflected path. However, in some cases where there are strong reflection in the environment, these cross terms cannot be ignored. An example of which is shown in Fig.~\ref{fig:beam_null_mot}. In this scenario, we beamform towards $0^\circ$ and add a delay of $d_\mathrm{obf} = 40 m$ to the direct path (green pattern) and simultaneously beamform towards the multipath at $-30^\circ$ (blue pattern). This creates a combined beamforming pattern (red) shown in the left inset. However, due to some side-lobe leakage in the direction of multipath and the presence of a strong reflector, we inadvertently add delay to the multipath as well. This creates a residual peak (in red dotted box) along with the delayed direct path peak (green box). This abnormal angle-distance profile will expose \name's spoofing and an attacker can potentially extract the correct direct path. 


\begin{figure}
\centering
\begin{minipage}{0.25\textwidth}
\captionsetup{width=0.78\textwidth}
\centering
   \includegraphics[width=0.8\linewidth]{figures/beam0_null_negative30.jpg} 
    \caption{Beamforming to 0 degree and nulling to -30 degree.}
    \label{fig:beam0null-30}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
\captionsetup{width=0.78\textwidth}
\centering
    \includegraphics[width=0.8\linewidth]{figures/beam_negative30_null0.jpg}
    \caption{Beamforming to -30 degree and nulling to 0 degree.}
    \label{fig:beam-30null0}
\end{minipage}
\end{figure}


\subsection{Nulled-Beamforming and Delaying}

To address the problem of imperfect beamforming that will also introduce inadvertent delay to the multipath, we propose nulled-beamforming and delaying method. The key idea is to mitigate the side-lobe leakage of the beamformed beams through nulling to the side-lobe direction. Specifically, when we beamform to the direct path, we will also null to the direction of the multipath to eliminate the effect of the side-lobe leakage on the multipath. As shown in Fig.~\ref{fig:beam0null-30}, the side-lobe effect at the nulling direction of -30 degree is minimum. Also, when we beamform to the multipath, we will null to the direction of the direct path to eliminate the effect of the side-lobe leakage on the direct path. As shown in Fig.~\ref{fig:beam-30null0}, the side-lobe effect at the nulling direction of 0 degree is minimum. As a result, when we add delay to the direct path, the multipath will barely be affected due to the nulling. 


To beamfrom towards the direct path while creating a null towards the multipath, we first need to obtain the null-space vectors of the multipath. Since the beamforming vector for multipath is $S_d(f_i, k)$, the null-space vectors of the multipath lie in $NULL(S_r(f_i, k))$ where $NULL(\cdot)$ indicates the null space. Let's assume the $j$-th nulling vector of the multipath is $nr_j(f_i,k)$, $j\in \{1, 2, 3, 4\}$, since the user has four antennas. Then, we use the weighted average of the null-space vectors as the precoding vector for the purpose of beamforming to the direct path and nulling to the multipath. Note, the weights for the linear combination of the null-space vectors are calculated based on the similarity of the multipath's null-space vector and the beamforming vector of the direct path. Specifically, since the beamforming vector of the direct path is $S_r(f_i, k)$, the $j$-th weight is caculated as $wd_j=S_d(f_i, k)^H nr_j(f_i,k)$ where $H$ indicates Hermitian. Then, the precoding vector for beamforming to the direct path and nulling to the multipath is obtained as follows:
\begin{equation}
    bdnr(f_i, k)=\frac{\sum_{j=1}^{4}wd_j nr_j(f_i,k)}{\sum_{j=1}^{4}wd_j}
\end{equation}
With the same insight, to beamform towards the multipath whiile create a null towards the direct path, the precoding vector can be obtained as follows:
\begin{equation}
        brnd(f_i, k)=\frac{\sum_{j=1}^{4}wr_j nd_j(f_i,k)}{\sum_{j=1}^{4}wr_j}
\end{equation}
where $wr_j=S_r(f_i, k)^H nd_j(f_i,k)$ indicates the $j$-th weight for null-space vector $nd_j(f_i,k)$ of the direct path. $nd_j(f_i,k)$ indicates $j$-th null-space vector of the direct path that lies in $NULL(S_d(f_i, k))$.


So far, we have had the precoding vector $ bdnr(f_i, k)$ for direct path and $brnd(f_i, k)$ for multipath. To achieve the goal of  AoA obfuscation, we need to only delay the direct path without affecting the multipath. To do so, our final precoding vector will be shown as follows:
\begin{equation}
    sv(f_i,k) = bdnr(f_i, k)e^{-j2\pi f_i\frac{d_\mathrm{obf}}{c}} + brnd(f_i, k)
\end{equation}

Thus, in \name we achieve ideal direct path obfuscation while minimizing the residual information of the obfuscation that could be identified by the attacker through our Nulled-Beamforming and Delay Algorithm.

==> design/design.tex <==
% !TEX root = paper.tex
\section{Design}\label{sec:design}
%\todo{are we giving away the idea too early?: yes, we want to make our idea clear at the beginning.}
In this section, we first illustrate an attack model which will violate the Wi-Fi user's location privacy. We then propose on how a straightforward idea of beam nulling to the direct path to protect the user's privacy comes at the cost of user's throughput degradation. Finally, we propose the design of \name for Wi-Fi user's location obfuscation, which makes the reflected path appear to be the direct path.

\subsection{Attack Model} 
The attacking Wi-Fi APs in an enterprise network (say a shopping mall) listen to the channel transmitted by the user and predict the user directions to each of the APs using state-of-the-art AoA algorithms (say SpotFi~\cite{spotfi}). The APs can use the AoAs either for
(a)`single-AP Localization' by using the ToF measurements (from Wi-Peep~\cite{wipeep} for example) for range and estimated AoA for direction, or (b) `Triangulation' by using AoAs across multiple APs to estimate user location. The AoA of the incoming Wi-Fi signal at the attacking AP can be extracted via Spotfi~\cite{spotfi} as shown in Fig.~\ref{fig:profiles}(a). As discussed, the direct path (green box) arrives earlier than the reflected path (blue box) and hence direct path's AoA can be reliably extracted even in multipath-rich environments. 

% \subsection{AoA-based Localization}\label{sec:design-aoa}

% Phase information has been widely used to accurately localize the Wi-Fi users, since it is more resilient to the noise in comparison to the signal strength. To be specific, the angle-of-arrival (AoA) information can be extracted based on the phase of the wireless channel. Let's assume the Wi-Fi AP has $N$ uniform linealy spaced antennas with antenna spacing $d$ of half wavelength $\lambda/2$, where $\lambda=c/f_c$. $c$ is the speed of light and $f_c$ is the center frequency. With the antenna array, the AoA can be computed with the following equation as shown in Fig.~\ref{fig:mirage-idea}(a).
% \begin{equation}
%     \label{eq:aoa}
%     \phi_{k}-\phi_{k-1}=\frac{2\pi}{\lambda} d\sin(\theta_d) = \pi \sin(\theta_d)
% \end{equation}
% where $\phi_k$ indicates the phase at $k$-th antenna, $\theta_d$ indicates the AoA of the direct path. However, in multipath-rich scenario, the Wi-Fi AP can observe multiple AoAs from different reflected paths. As the signals from the direct path will travel shorter distance than the other multipath, we can identify the AoA from the direct path with the shortest time of flight. Combining this AoA information from at least two AP's will allow us to triangulate the user's location. 

% With AoA information at one WiFi AP, we can know the direction of the WiFi user in comparison to the WiFi AP. To localize the WiFi user, we need to have at least AoA information to triangulate the WiFi user. 


%Though as stated earlier predicting AoA of the user is more robust and accurate than the timing estimates of the 

%We can create a simple null in the direction of the attacker using the downlink channel measurements. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/results.pdf}
    \caption{Angle-Distance profiles representing the direct path and reflected path angle of arrivals and their relative distance travelled. Measurement from COTS AP in (a) without \name, in (b) with nulling the direct path, in (c) with \name obfuscation applied.}
    \label{fig:profiles}
\end{figure}



\subsection{Nulling to the Direct Path}
\label{sub:nulling}
%\todo{add more info on how nulling is done? yes.}
%\todo{refer to figures better, will do}
Hence, to obfuscate the AoA information at the Wi-Fi user, a straightforward idea is to null this direct path to the AP. That is the user can beamform such that there is a null in the beampattern in the direction of AP's direct path. Now the attacker Wi-Fi AP will only observe the multipath and regard it as the direct path for localization. To perform this nulling, the Wi-Fi user extracts the AoA of direct path (i.e., $\theta_d$) and AoA of the earliest reflected path (i.e., $\theta_r$) from a downlink (AP to user) channel measurement. For the sake of simplicity, we only consider two paths. To null the direct path, the Wi-Fi user needs to apply the beamforming weights $N_d(f_i,k)$ to their data streams to null in the $\theta_d$ direction, where $i$ indicates the subcarrier index and $k$ indicates the antenna index. After we `precode' the data stream $X(f_i, k)$ with nulling weights, the Wi-Fi AP will receive the following signals:
\begin{align*}
    Y(f_i,k) &=H(f_i,k)N_d(f_i, k)X(f_i,k)\\
             &=(H_d(f_i, k)+H_r(f_i,k))N_d(f_i, k)X(f_i,k)\\
             &= H_r(f_i,k)N_d(f_i, k)X(f_i,k)
\end{align*}
where $Y(f_i,k)$ and $H(f_i,k)$ indicate the received signal and wireless channel on $k$-th antenna and $f_i$ subcarrier. $H(f_i,k)=H_d(f_k, k)+H_r(f_i,k)$ where $H_d$ and $H_r$ indicate the direct path and  reflected path wireless channel. Note that $H_d(f_i, k)N_d(f_i,k)=0$ as $N_d(f_i,k)$ is chosen to lie in the null space of $H_d(f_i, k)$ \cite{li2005null}. The Wi-Fi AP will estimate the wireless channel as $H_r(f_i,k)N_d(f_i, k)$, which only contains the reflected path, thereby preventing the attacker from extracting the direct path AoA. 

This is illustrated in the angle-distance profile in Fig.~\ref{fig:profiles}(b). Note the reduced power of the direct path. However, this simple idea has two key flaws. First, nulling to the direct path will decrease the signal strength at the Wi-Fi AP and degrade the network throughput. Second, in case the nulling angle is predicted incorrectly by the user, nulling will be ineffective and a residual peak of the direct path will remain exposing the user's location. Clearly, this solution is impractical and we propose \name for user location obfuscation to eliminate this side-effect.

\subsection{Beamforming and Delaying}\label{sec:mirage-des}

To overcome this user's throughput degradation we need to ensure the direct path is preserved, as direct-path contributes to majority of the channel diversity. However the presence of the direct path will appear as a strong signal at the Wi-Fi AP and an attacker can easily extract the AoA. However, to disambiguate the effects of the inevitable reflected paths, the attacker relies on the simple heuristic that the direct path always travels the shortest path. Specifically, for a distance travelled $d$, the phases accumulated across the various subcarriers are given by $e^{-2\pi f_c \frac{d}{c}}$. By leveraging super-resolution localization algorithms~\cite{spotfi}, the attacker can hence separate the various paths in the time-domain and predict the direct path. 

Here we provide a key insight -- delaying only the direct path signal invalidates the foundational heuristic to select the correct AoA. With this in mind, we propose to beamform to direct path and multipath and add delay to the direct path. This ensures communication throughput will be preserved over the beamforming and the user's location will be obfuscated through adding the delay to the direct path. This is qualitatively illustrated in Fig.~\ref{fig:profiles}(c). The Wi-Fi user adds a delay of $15$ m in the direction of the direct path and successfully pushes the direct path peak (green box) predicted by SpotFi to the right of the multipath peak (blue box).    

%\todo{why is adding $\tau$ in the manner shown make sense? it's not clear}: will be more explanation
%\todo{how is $\tau$ chosen? } depends on user's expectation so it is empirical

\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.40\linewidth}
    \includegraphics[width=\linewidth]{figures/setup.pdf}
    \subcaption{}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
        \begin{tabular}{|c|c|c|cccc|}
        \hline
        \multirow{2}{*}{} &
          \multirow{2}{*}{No obf.} &
          \multirow{2}{*}{Nulling} &
          \multicolumn{4}{c|}{\name with delay of} \\ \cline{4-7} 
         &  &  & \multicolumn{1}{c|}{0 (m)} & \multicolumn{1}{c|}{20 (m)} & \multicolumn{1}{c|}{30 (m)} & 40 (m) \\ \hline
        AoA error &
          $0^\circ$ &
          $62^\circ$ &
          \multicolumn{1}{c|}{$0^\circ$} &
          \multicolumn{1}{c|}{$58^\circ$} &
          \multicolumn{1}{c|}{$61^\circ$} &
          $53^\circ$ \\ \hline
        \begin{tabular}[c]{@{}c@{}}RSSI\\ (dBm)\end{tabular} &
          -65 &
          -71 &
          \multicolumn{1}{c|}{-64} &
          \multicolumn{1}{c|}{-64} &
          \multicolumn{1}{c|}{-64} &
          -62 \\ \hline
        \end{tabular}
        \subcaption{}
        \label{table:aoa_rssi}
    \end{minipage}
    \caption{\textbf{(a)} Hardware setup showcasing the ASUS WiFi-AP, WARP client and reflector. (b) AoA error and RSSI measured without obfuscation; with nulling; and using \name to delay the path by varying amounts}
    \label{fig:example-result}
\end{figure*}


Specifically, to beamform to the direct path and multipath, we need to have the beamforming vector $S_d(f_i,k)$ and $S_r(f_i,k)$ for the direct path and reflected path respectively~\cite{beam_forming_doc}. The specific beamforming angles are predicted via a downlink channel measurement at the user. Hence, the Wi-Fi user will use the precoding weight of $S_d(f_i,k)e^{-j2\pi f_i d_\mathrm{obf}/c}+S_r(f_i,k)$, where $d_\mathrm{obf}$ indicates the additional path length that Wi-Fi user wants to add to obfuscate its location for Wi-Fi AP as shown in Fig.~\ref{fig:mirage-idea}(d). We ensure that $d_\mathrm{obf} > d_\mathrm{multipath} - d_\mathrm{direct}$ via the same downlink channel measurements. Then, the Wi-Fi AP will receive the following signals:
\begin{align}
\label{eq:beam:delay}
     Y(f_i, k)&=H(f_i,k)(S_d(f_i,k)e^{-j2\pi f_i \frac{d_\mathrm{obf}}{c}} + S_r(f_i,k))X(f_i,k)\nonumber \\
             &=(H_d(f_k, k)+H_r(f_i,k))(S_d(f_i,k)e^{-j2\pi f_i\frac{d_\mathrm{obf}}{c}}\nonumber \\
             & \quad \quad \quad \quad  + S_r(f_i,k))X(f_i,k)\nonumber\\
             &=(H_d(f_k, k)S_d(f_i,k)e^{-j2\pi f_i\frac{d_\mathrm{obf}}{c}} \nonumber\\
             & \quad \quad \quad \quad + H_r(f_i,k)S_r(f_i,k))X(f_i,k)
\end{align}
Beamforming in the directions of the direct path ensures weaker energy directed towards strongest multipath and vice versa. Hence, in Eqn.~\ref{eq:beam:delay}, the cross terms $H_d(f_k, k)S_r(f_i,k)$ and $H_r(f_i,k)S_d(f_i,k)e^{-j2\pi f_i d_\mathrm{obf}/c}$ are ignored. Thus, the wireless channel is $H_d(f_k, k)S_d(f_i,k)e^{-j2\pi f_i d_\mathrm{obf}/c}+H_r(f_i,k)S_r(f_i,k)$, which will only contain direct path with delay of $d_\mathrm{obf}$ and multipath without any delay. 


% will be negligible and ignored due to the beamforming weights. Specifically, the beamforming weights $S_r$ for multipath will have large angle relative to the direct-path wireless channel $H_d$, since $S_r(f_i,k)$ is the beamforming weight for multipath. So, $H_d(f_k, k)S_r(f_i,k)$ will become small. Similarly, the beamforming weight of $S_d(f_i,k)$ will also have large angle relative to the multipath wirless channel $H_r(f_i,k)$, since $S_d(f_i,k)$ is the beamforming weight for the direct path. So, $H_r(f_i,k)S_d(f_i,k)$ will become small. As a result, the cross terms will comparably small in comparison to the remaining terms in Equation~\ref{eq:beam:delay}. 



%\subsection{Beam-Nulling}
%The idea is to perform digital beamforming to create a NULL in the direction of the AP.
%While, this would work for signals with signal strength of around 40-50dB, as reduction of the snr by blocking the direct path would make the signal strength to about 20dB, which still doesn't affect the throughput of the network.

%The idea of such digital beamforming based nulling would not work for signals that are already around 20dB would be seriously affected and thus limiting network throughput.

%\subsection{Create \name:}

%The idea comes from the assumption that AoA algorithms depend on, that is the `direct path is the shortest path'.

%This has a flaw if we can ensure the phase corresponding to the direct path is delayed such that the multipath appears before the direct path.

%We can do that by digital beamforming.

%\todo{What are the challenges for this digital beamforming?}

%\subsection{Dealing with Dynamic Multipath}

%How do we do this?

%\subsection{Can the user still decode their Location?}

%Have to maybe propose or at-least say something on the user can maybe decode their location if they wanted it from the downlink channel measurements they have received.https://www.overleaf.com/project/633ba450dbdc3679eab86e10

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/discussion.pdf}
    \vspace{1pt}
    \caption{Imperfect beamforming introduces residual peak in angle-distance profile (red dotted box) due to the power leakage from the side lobe of the direct path beamforming. \textit{(left inset)} Antenna beamforming patterns transmitted by the user; \textit{right inset} received SpotFi profile at a commodity Wi-Fi AP}
    \label{fig:beam_null_mot}
\end{figure*}

\subsection{Problem of Imperfect Beamforming}

We have demonstrated \name's obfuscation for the Wi-Fi user's location through beamforming and delaying through a few examples. However in \name's design we make a critical assumption. We ignore the cross terms in Eqn.~\ref{eq:beam:delay} when adding delay to the direct path due to weaker energy directed towards the reflected path. However, in some cases where there are strong reflection in the environment, these cross terms cannot be ignored. An exemplary case is shown in Fig.~\ref{fig:beam_null_mot}. In this scenario, we beamform towards $0^\circ$ and add a delay of $d_\mathrm{obf} = 40 m$ to the direct path (green pattern) and simultaneously beamform towards the multipath at $-30^\circ$ (blue pattern). This creates a combined beamforming pattern (red) shown in the left inset. However, due to some side-lobe leakage in the direction of multipath and the presence of a strong reflector, we inadvertently add delay to the multipath as well. This creates a residual peak (in red dotted box) along with the delayed direct path peak (green box). This abnormal angle-distance profile will expose \name's spoofing and an attacker can potentially extract the correct direct path. 


\begin{figure}
\centering
\begin{minipage}{0.25\textwidth}
\captionsetup{width=0.78\textwidth}
\centering
   \includegraphics[width=0.8\linewidth]{figures/beam0_null_negative30.jpg} 
    \caption{Beamforming to 0 degree and nulling to -30 degree.}
    \label{fig:beam0null-30}
\end{minipage}%
\begin{minipage}{0.25\textwidth}
\captionsetup{width=0.78\textwidth}
\centering
    \includegraphics[width=0.8\linewidth]{figures/beam_negative30_null0.jpg}
    \caption{Beamforming to -30 degree and nulling to 0 degree.}
    \label{fig:beam-30null0}
\end{minipage}
\end{figure}


\subsection{Beamforming, Nulling and Delaying}

To address address the problem of imperfect beamforming that will also introduce inadvertent delay to the multipath, we propose beamforming, nulling and delaying method. The key idea is to mitigate the side-lobe leakage through nulling to the side-lobe direction. Specifically, when we beamform to the direct path, we will also null to the direction of the multipath to eliminate the effect of the side-lobe leakage on the multipath. As shown in Fig.~\ref{fig:beam0null-30}, the side-lobe effect at the nulling direction of -30 degree is minimum. Also, when we beamform to the multipath, we will null to the direction of the direct path to eliminate the effect of the side-lobe leakage on the direct path. As shown in Fig.~\ref{fig:beam-30null0}, the side-lobe effect at the nulling direction of 0 degree is minimum. As a result, when we add delay to the direct path, the multipath will barely be affected due to the nulling. 


To beamfrom to direct path and null to the multipath, we first need to obtain the nulling vectors of the multipath. Since the beamforming vector for multipath is $S_d(f_i, k)$, the nulling vectors of the multipath lie in $NULL(S_r(f_i, k))$ where $NULL(\cdot)$ indicates the null space. Let's assume the $j$-th nulling vector of the multipath is $nr_j(f_i,k)$, $j\in \{1, 2, 3, 4\}$, since the user has four antennas. Then, we use the weighted average of the nulling vectors as the precoding vector for the purpose of beamforming to the direct path and nulling to the multipath. Note, the weights are calculated based on the similarity of the nulling vector and the beamforming vector of the direct path. Specifically, since the beamforming vector of the direct path is $S_r(f_i, k)$, the $j$-th weight is caculated as $wd_j=S_d(f_i, k)^H nr_j(f_i,k)$ where $H$ indicates Hermitian. Then, the precoding vector for beamforming to the direct path and nulling to the multipath is obtained as follows:
\begin{equation}
    bdnr(f_i, k)=\frac{\sum_{j=1}^{4}wd_j nr_j(f_i,k)}{\sum_{j=1}^{4}wd_j}
\end{equation}
With the same insight, to beamform to the multipath and null to the direct path, the precoding vector can be obtained as follows:
\begin{equation}
        brnd(f_i, k)=\frac{\sum_{j=1}^{4}wr_j nd_j(f_i,k)}{\sum_{j=1}^{4}wr_j}
\end{equation}
where $wr_j=S_r(f_i, k)^H nd_j(f_i,k)$ indicates the $j$-th weight for nulling vector $nd_j(f_i,k)$ of the direct path. $nd_j(f_i,k)$ indicates $j$-th nulling vector of the direct path that lies in $NULL(S_d(f_i, k))$.



So far, we have had the precoding vector $ bdnr(f_i, k)$ for direct path and $brnd(f_i, k)$ for multipath. To achieve the goal of  AoA obfuscation, we need to only delay the direct path without affecting the multipath. To do so, our final precoding vector will be shown as follows:
\begin{equation}
    sv(f_i,k) = bdnr(f_i, k)e^{-j2\pi f_i\frac{d_\mathrm{obf}}{c}} + brnd(f_i, k)
\end{equation}
